Enhancing Autonomous Driving Systems with On-Board Deployed Large Language Models

Neural Networks (NNs) trained through supervised learning struggle with managing edge-case scenarios common in real-world driving due to the intractability of exhaustive datasets covering all edge-cases, making knowledge-driven approaches, akin to how humans intuitively detect unexpected driving behavior, a suitable complement to data-driven methods. This work proposes a hybrid architecture combining low-level Model Predictive Controller (MPC) with locally deployed Large Language Models (LLMs) to enhance decision-making and Human Machine Interaction (HMI). The DecisionxLLM module evaluates robotic state information against natural language instructions to ensure adherence to desired driving behavior. The MPCxLLM module then adjusts MPC parameters based on LLM-generated insights, achieving control adaptability while preserving the safety and constraint guarantees of traditional MPC systems. Further, to enable efficient on-board deployment and to eliminate dependency on cloud connectivity, we shift processing to the on-board computing platform: We propose an approach that exploits Retrieval Augmented Generation (RAG), Low Rank Adaptation (LoRA) fine-tuning, and quantization. Experimental results demonstrate that these enhancements yield significant improvements in reasoning accuracy by up to 10.45%, control adaptability by as much as 52.2%, and up to 10.5x increase in computational efficiency (tokens/s), validating the proposed framework's practicality for real-time deployment even on down-scaled robotic platforms. This work bridges high-level decision-making with low-level control adaptability, offering a synergistic framework for knowledge-driven and adaptive Autonomous Driving Systems (ADS).

==> ext_tables/ext_tables_compute.tex <==
\begin{table}[!htb] % here, top, bottom, page (float page)
\small
    \centering % Ensures that the table is centered in the text column
    % \resizebox{\textwidth}{!}{%
    \setlength{\tabcolsep}{0.7 mm}
    \begin{tabular}{l|l|c|c|c|c|c|cc}
    \toprule
    \textbf{HW} & \textbf{LLM} & \textbf{Quant} & \textbf{Param} & \textbf{Mem} & \textbf{Tokens} & \textbf{Tokens/s} & \multicolumn{2}{c}{\textbf{Time [s]}$\downarrow$} \\
    & & & \textbf{[\#B]} & \textbf{[GB]} & \textbf{[\#]} & \textbf{[s$^{-1}$]$\uparrow$} & $\mu_{t}$ & $\sigma_{t}$ \\
    \midrule
    RTX & Phi3 & FP16 & 3.8 & 4.3 & 72 & \textbf{25.23} & \textbf{2.85} & \textbf{0.05} \\
    3090 & Phi4  & FP16 & 14 & 10.9 & 140 & 10.14 & 13.8 & 0.09 \\
    & Qwen  & FP16 & 7 & 7.8 & 50 & 11.14 & 4.51 & 0.08 \\
    \cmidrule{2-9}
    & Phi3 & Q5 & 3.8 & 3.9 & 110 & \textbf{148.36} & \textbf{0.75} & \textbf{0.06} \\
    & Qwen  & Q5 & 7 & 5.6 & 97 & 107.52 & 0.91 & 0.08 \\
    \midrule
    \multirow{3}{*}{\tabincell{l}{Jetson\\Orin\\AGX}} & Phi3 & FP16 & 3.8 & 4.2 & 72 & \textbf{4.71} & \textbf{15.29} & \textbf{0.48} \\
    & Qwen  & FP16 & 7 & 6.9 & 64 & 2.11 & 30.48 & 0.59 \\
    \cmidrule{2-9}
    & Phi3 & Q5 & 3.8 & 3.6 & 154 & \textbf{32.47} & \textbf{4.80} & \textbf{0.58} \\
    & Qwen  & Q5 & 7 & 5.3 & 121 & 22.12 & 5.52 & \textbf{0.58} \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of computational performance for locally deployable models, \textit{Phi3-mini-3.8b}, \textit{Phi4-14b} and \textit{Qwen2.5-7b}. The \glspl{llm} were deployed on both an RTX 3090 GPU and the \textit{Jetson Orin AGX} robotic \gls{obc}. FP16 denotes full-precision models, while Q5 represents the \texttt{Q5\_k\_m} quantized models implemented via the \texttt{llama.cpp} inference engine. The number of tokens denotes the output tokens generated for the given inference.}
    \label{tab:compute}
\end{table}

Given the need for efficient hardware utilization in autonomous driving scenarios and the necessity for real-time interaction, the efficiency based on two models is evaluated and discussed for the locally deployable \textit{Phi3-mini-3.8b} and \textit{Qwen2.5-7b} (\Cref{tab:compute}). \textit{Phi4-14b} is only run on the RTX 3090 with FP16, due to the \gls{llm} not being able to run within the proposed frameworks quantized pipeline due to the model just being released, and secondly due to the relatively low inference speed compared to the other tested \glspl{llm}.

For the framework based on Phi3, when deployed on RTX 3090 hardware using FP16, the model with 3.8 billion parameters achieves a token output rate of 25.23 tokens per second and utilizes 4.3 GB of memory. In contrast, when quantized to \texttt{Q5\_k\_m}, the memory usage decreases to 3.9 GB, and the throughput speed significantly increases to 148.36 tokens per second. On the computationally constrained Jetson Orin hardware, the FP16 Phi3 manages an inference time of 15.29 seconds, while the \texttt{Q5\_k\_m} quantized model shows improved performance with an inference time of 4.80 seconds for 154 tokens.
For the framework based on Qwen, the outcome is similar. On the RTX 3090, when the model is quantized to \texttt{Q5\_k\_m}, the throughput speed rises to nearly 9.7$\times$ that of FP16, reaching 107.52 tokens per second. Thus, the inference time decreases significantly to 0.91 seconds, approximately 20\% of the time required for FP16. On the \textit{Jetson Orin}, the \texttt{Q5\_k\_m} configuration increases the throughput to about 10.5$\times$ compared to the FP16, at 22.12 tokens per second. The inference time is lowered to 5.52 seconds, less than 20\% of that of the FP16.

These results highlight the substantial efficiency gains achievable through post-training quantization, enabling the deployment of our \glspl{llm}-based framework in computationally constrained hardware while maintaining real-time capabilities on robotic platforms.

==> ext_tables/ext_tables_decision.tex <==
\begin{table}[!htb] % here, top, bottom, page (float page)
    \centering % Ensures that the table is centered in the text column
    \begin{adjustbox}{max width=\columnwidth}
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{LLM} & \textbf{Quant} & \textbf{LoRA} & \textbf{RAG} & \textbf{Accuracy [\%]}\bm{$\uparrow$}\\
    \midrule
    GPT4o & ? & \xmark & \xmark & \textbf{81.68} \\
    Phi3-mini & FP16 & \xmark & \xmark & 72.15 \\
    Phi4 & FP16 & \xmark & \xmark & 75.79 \\
    Qwen-7b & FP16 & \xmark & \xmark & 77.75\\
    \midrule
    GPT4o & ? & \xmark & \cmark & \textbf{92.48} \\
    Phi3-mini & FP16 & \xmark & \cmark & 78.69 \\
    Phi4 & FP16 & \xmark & \cmark & 81.99 \\
    Qwen-7b & FP16 & \xmark & \cmark & 82.47 \\
    \midrule
    Phi3-mini & FP16 & \cmark & \cmark & 82.60 \\
    Phi4 & FP16 & \cmark & \cmark & \textbf{89.83} \\
    Qwen-7b & FP16 & \cmark & \cmark & 87.32 \\
    \midrule
    Phi3-mini & Q5 & \cmark & \cmark & 84.95 \\
    Qwen-7b & Q5 & \cmark & \cmark & \textbf{87.02} \\
    \bottomrule
    \end{tabular}%
    \end{adjustbox}
    \caption{Decision-making accuracy across various \glspl{llm}, illustrating the impact of quantization, \gls{lora} fine-tuning, and \gls{rag} on the performance of the \textit{DecisionxLLM} module in evaluating whether a robotic state aligns with desired driving behavior. Higher accuracy values indicate improved adherence to the specified driving characteristics. ? indicates that this is proprietary knowledge, not known to the public.}
    \label{tab:decision_res}
\end{table}


\Cref{tab:decision_res} demonstrates the performance of the \textit{DecisionxLLM} module in determining whether a robotic state adheres to the desired human driving behavior. All performance improvements are stated in absolute percentage points. The results indicate that the inclusion of \gls{rag} consistently enhances model performance across all tested \glspl{llm}, with an average improvement of 7.07\% (\textit{GPT4o/Phi3/Phi4/Qwen2.5} -- +10.8/+6.54/+6.2/+4.72\%). 
Fine-tuning locally deployable \glspl{llm} via \textit{GPT4o} distillation, as detailed in \Cref{subsec:finetuning}, further improves model accuracy by an average of 5.53\% (\textit{Phi3/Phi4/Qwen2.5} -- +3.91/+7.84/+4.85\%). 
Lastly, quantization, which is essential for deployment on computationally constrained \glspl{obc}, does not substantially degrade decision-making performance, maintaining accuracy within a margin of 1.02\% relative to full-precision models (\textit{Phi3/Qwen2.5} -- +2.35/-0.3\%). \textit{Phi4} however, was not able to be run within the quantized pipeline due to the low amount of time since it's release.

In summary, the proposed system effectively reasons over robotic state information conditioned on human driving instructions, benefiting from \gls{rag}, \gls{lora} fine-tuning (\textit{Phi3/Phi4/Qwen2.5} -- +10.45/+14.04/+9.57\%), and demonstrating resilience to the effects of model quantization for local deployment. Further, comparing the two local \glspl{llm}, \textit{Qwen2.5-7b} consistently outperforms \textit{Phi3-mini-3.8b} across all settings, making it the preferred choice. That said, \textit{GPT4o} achieves the highest performance overall, and the framework's flexibility enables its use in scenarios where dependency on cloud connectivity is warranted.

==> ext_tables/ext_tables_mpc.tex <==
\begin{table*}[!htb] % here, top, bottom, page (float page)
    \centering % Ensures that the table is centered in the text column
    %\resizebox{\textwidth}{!}{%
    \begin{tabular}{l|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{LLM} & \textbf{Quant} & \textbf{LoRA} & \textbf{RAG} & \bm{$E_C [m]\downarrow$} & \bm{$E_V [ms^{-1}]\downarrow$} &  \bm{$E_R [ms^{-1}]\downarrow$} & \bm{$E_S [ms^{-2}]\downarrow$} & \textbf{Improve [\%]}\bm{$\uparrow$} \\
    \midrule
    \gls{mpc} (baseline) & - & - & - & 0.7 & 1.6 & 4.6 & 1.5 & - \\
    \midrule
    GPT4o & ? & \xmark & \xmark & \textbf{0.5 (19.3\%)} & 1.8 (-11.8\%) & 1.5 (68.1\%) & 1.4 (5.1\%) & 20.2\% \\
    Phi3-mini & FP16 & \xmark & \xmark & N.C. & 1.9 (-17.1\%) & 2.8 (39.5\%) & 11.8 (-711.4\%) & -229.6\%$^\dagger$ \\
    Phi4 & FP16 & \xmark & \xmark & 0.6 (8.7\%) & \textbf{0.9 (43.9\%)} & 1.8 (61.1\%) & \textbf{1.2 (19.3\%)} & \textbf{33.3\%} \\
    Qwen-7b & FP16 & \xmark & \xmark & 0.7 (-14.6\%) & 1.8 (-14.4\%) & \textbf{1.3 (70.9\%)} & 2.0 (-40.4\%) & 0.5\% \\
    \midrule
    GPT4o & ? & \xmark & \cmark & 0.5 (21.3\%) & 0.3 (81.5\%) & \textbf{1.2 (74.7\%)} & 1.3 (7.5\%) & \textbf{46.3\%} \\
    Phi3-mini & FP16 & \xmark & \cmark & 0.6 (6.6\%) & 0.6 (60.8\%) & 4.2 (9.8\%) & \textbf{0.3 (82.5\%)} & 39.9\% \\
    Phi4 & FP16 & \xmark & \cmark & \textbf{0.4 (43.3\%)} & 0.2 (86.0\%) & 2.7 (41.1\%) & 1.3 (7.5\%) & 44.4\% \\
    Qwen-7b & FP16 & \xmark & \cmark & 0.6 (8.6\%) & \textbf{0.1 (91.7\%)} & 1.5 (67.7\%) & 1.4 (4.8\%) & 43.2\% \\
    \midrule
    Phi3-mini & FP16 & \cmark & \cmark & 0.7 (-0.3\%) & 0.6 (59.3\%) & 1.0 (78.8\%) & \textbf{0.8 (42.8\%)} & 45.1\% \\
    Phi4 & FP16 & \cmark & \cmark & 0.4 (35.6\%) & 0.4 (\textbf{75.1\%)} & \textbf{0.9 (80.3\%)} & 1.3 (11.9\%) & 50.7\% \\
    Qwen-7b & FP16 & \cmark & \cmark & \textbf{0.4 (37.2\%)} & 0.4 (71.9\%) & 1.1 (76.4\%) & 1.1 (23.2\%) & \textbf{52.2\%} \\
    \midrule
    Phi3-mini & Q5 & \cmark & \cmark & 0.57 (12.6\%) & 0.5 (70.7\%) & 1.2 (73.6\%) & 1.1 (-22.3\%) & 44.\% \\
    Qwen-7b & Q5 & \cmark & \cmark & \textbf{0.43 (33.4\%)} & \textbf{0.2 (85.8\%)} & \textbf{1.3 (71.3\%)} & \textbf{1.5 (-3.3\%)} & \textbf{46.8\%} \\
    \bottomrule
    \end{tabular}%8
    %}
    \caption{Quantitative Comparison of \gls{llm} configurations with \gls{mpc}. Performance metrics include deviation from the centerline ($E_C [m]$), reference velocity ($E_V [ms^{-1}]$), reversing accuracy ($E_R [ms^{-1}]$), and driving smoothness ($E_S [ms^{-2}]$), with percentage improvements shown relative to the \gls{mpc} baseline. The average improvement column summarizes overall performance across all metrics. $\dagger$ indicates an average over completed runs, excluding N.C. (\textit{Not Completed}). ? indicates that this is proprietary knowledge, not known to the public.}
    \label{tab:control_res}
\end{table*}


\subsection{MPCxLLM --- Control Adaptability} \label{subsec:results_mpcxllm}
The \textit{MPCxLLM} module is evaluated, in a closed-loop simulation environment of the open-source \textit{F1TENTH} autonomy stack \cite{forzaeth}, where the \gls{mpc} handles vehicle control. In this context, simulation is preferred over physical testing due to time efficiency and access to ground-truth data.

The \gls{llm} governs interaction scenarios to enable the computation of quantifiable \gls{rmse} metrics. We assess changes in closed-loop behavior relative to the default \gls{mpc} formulation outlined in \Cref{subsec:mpc}, using the following criteria:

\begin{enumerate}[I] 
    \item \textbf{Centerline:} \gls{rmse} of the distance from the centerline, denoted as $E_C [m]$. Instruction prompt: "Drive as far away from the walls as possible!"
    \item \textbf{Reference Velocity:} \gls{rmse} deviation from a human-provided reference velocity, denoted as $E_V [ms^{-1}]$.  Instruction prompt: "Follow the reference velocity of 1.25 m/s as closely as possible!"
    \item \textbf{Reversing:} \gls{rmse} deviation from a negative reference velocity specified by the human, denoted as $E_R [ms^{-1}]$. Instruction prompt: "Drive the track in reverse at -1 m/s!"
    \item \textbf{Smooth Driving:} \gls{rmse} of acceleration deviating from 0 $ms^{-2}$, denoted as $E_S [ms^{-2}]$. Instruction prompt: "Reduce jerkyness!"
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%% Start Group MPC bubbles %%%%%%%%%%%%%%%%%%%%%%%%%
% User Instruction Bubble
\begin{mpcbubble}{2a}{Instruction}
Reverse the car!
\end{mpcbubble}

% MPC Prompt Bubble
\begin{mpcbubble}{2b}{Prompt}
Adapt the tuneable parameters of the MPC so that the car achieves the following: \texttt{instruction}.\\
This is the MPC formulation: \texttt{base\_memory}.\\
Make use of these memories: \texttt{rag\_memories}.\\
Return format:\\
\texttt{new\_mpc\_params} = \texttt{\{param1: new\_value1, param2: new\_value2, ...\}}
\end{mpcbubble}

% MPC Output Bubble
\begin{mpcbubble}{2c}{Response}
\texttt{new\_mpc\_params} = \texttt{ \{qv: 0.1, 'qn': 40, qalpha: 50, ddelta\_min: -5,
ddelta\_max: 0, dv\_min: -50, dv\_max: -1, v\_min: -1, v\_max: -1, boundary\_inflation: 0.1\} }\\
\textbf{Explanation:} The new parameters are tuned to achieve the goal of driving the track in reverse at -1.0 m/s. The minimum and maximum velocities (\texttt{v\_min} and \texttt{v\_max}) are set to -1 and -1, respectively, to ensure the velocity is at -1.0 m/s.
\end{mpcbubble}
\setcounter{bubblegroup}{2}
%%%%%%%%%%%%%%%%%%%%%%%%%% End Group MPC bubbles %%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[height=5cm]{figs/wall_clearance-compressed.pdf}
        \caption{Prompt: \emph{"Drive further away from the wall."}}
        \label{fig:robot_centerline}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[height=5cm]{figs/crash_recovery-compressed.pdf}
        \caption{Prompt: \emph{”Drive normally!”}}
        \label{fig:robot_crash_recovery}
    \end{subfigure}
    \caption{Visualization of physical robot behaviors: (a) maintaining clearance from walls, (b) recovering from a crash scenario. All experiments were performed utilizing the edge-deployed \textit{Qwen2.5-7b} \gls{llm}.}
    \label{fig:robot_res}
\end{figure*}


It is important to note that while the evaluation scenarios presented here are specifically designed to ensure the computation of quantifiable metrics, such as \gls{rmse}, the \textit{MPCxLLM} module is capable of processing and responding to a wide range of other natural language instructions. The chosen scenarios are simply representative examples where measurable outcomes --- like centerline deviation, velocity tracking, and smooth driving --- allow for clear and reproducible analysis. However, the methodology and interaction flow described are not limited to these examples and can extend to other instructions.

\Cref{tab:control_res} demonstrates the controller adaptability through the evaluated \glspl{llm}. The \gls{mpc} baseline, represents the different \glspl{rmse} adherences with default parameters, tuned for nominal operation of the vehicle. All percentage improvements are reported in absolute percentage points. The results show that the inclusion of \gls{rag} generally improves instruction adherence for locally deployable \glspl{llm} (\textit{Phi3-mini, Phi4,+  Qwen2.5}) by approximately 31\%, although performance without \gls{rag} can be negligible or even detrimental. \textit{GPT4o} cannot be deployed via \gls{lora} fine-tuning and is therefore excluded. For locally deployable models, \gls{lora} fine-tuning offers an additional 15–20\% improvement over \gls{rag}-only setups. Hence, in terms of controller adaptability, both \gls{rag} and \gls{lora} demonstrate a 45.1\%, 50.7\%, and 52.2\%  (for \textit{Phi3-mini}, \textit{Phi4}, and \textit{Qwen2.5} respectively) improvement over the nominal \gls{mpc} baseline. Lastly, quantization introduces a minor ~1-6\% performance drop but remains essential for achieving acceptable computational performance on the \gls{obc}, as detailed in \Cref{subsec:results_compute}. Again, the \textit{Phi4} \gls{llm} was not able to be run within the quantization pipeline due to time reasons. Note that the numerical values should be interpreted with caution, as the closed-loop experiment is not deterministic, since it depends on the \gls{mpc}'s adherence quality and the specific map used in the open-source simulation environment \cite{forzaeth}, hence the relative improvement should be regarded. From the local and quantized \glspl{llm}, \Cref{tab:control_res} shows that \textit{Qwen2.5-7b} consistently outperforms \textit{Phi3-mini-3.8b} in terms of controller adaptability.

\Cref{bubble:2a} illustrates a qualitative result of the \textit{MPCxLLM} module. The input instruction is passed to the \gls{llm}, where the prompt demonstrates how the \gls{llm} is guided by the instruction and optionally enriched by the \textit{MPCxLLM} \gls{rag}. Finally, the module's output displays a new set of \gls{mpc} cost and constraint parameters that are subsequently parsed and transmitted to the \gls{mpc} as a \gls{ros} dynamic reconfigurable parameter.

